On the Non-Relativistic Groundstate Energy of Positronium in Relativistic Schroedinger Theory

The \emph{Relativistic Schr\"odinger Theory} (RST) has been set up as an alternative form of particle theory. This theory obeys the fundamental symmetries which are required to hold for any meaningful theory: gauge and Lorentz covariance (RST can be formulated even over a pseudo-Riemannian space-time). But the question is now whether obeying those fundamental symmetries is sufficient for the practical success of a theory, i.e. whether the predictions are in agreement with the experimental findings. In this context, the non-relativistic energy spectrum of positronium has been considered in some precedent papers. Here, the problem is that exact solutions of the RST eigenvalue system cannot be obtained and one has to resort to approximate solutions. For this purpose, a variational method is applied in the present paper which yields the RST groundstate energy smaller than the former results and than its conventional counterpart by some 10\%. Such deviations are also observed when one compares the approximate RST spectrum (up to quantum numbers $n\approx 100$) to the corresponding predictions of the conventional theory. It seems presently not possible to decide whether those deviations are due to RST itself or are merely due to the applied approximation technique. Thus the practical usefulness of RST must remain unclarified for the moment.

==> app.tex <==
\subsection*{Appendix}

\centerline{\large \bf \emph{Trial Ansatz~$\overset{\circ}{\Psi}{}^{\{0\}}_\infty(y)$ with vanishing
Derivative at the Origin}}
\vspace*{5mm}

The set of trial ans\"atze~$\Psi{}^{\{0\}}_\infty(y)$~(40) with variational parameter g
contains indeed a member~($\overset{\circ}{\Psi}{}^{\{0\}}_\infty(y)$, say) which has
vanishing derivative at the origin
\begin{equation}
  \label{eq:a1}
  \frac{d \overset{\circ}{\Psi}{}^{\{0\}}_\infty(y)}{dy} = 0\ .
\end{equation}
This specific member is characterized through a special value~($\overset{\circ}{g}$) of
the variational parameter~$g$
\begin{equation}
  \label{eq:a2}
  g \Rightarrow \overset{\circ}{g} = \ln 2 \ .
\end{equation}
But this member carries slightly higher energy than the optimal member which
has \mbox{$g\Rightarrow g_*=-0,71819\ldots$ (Fig.1)}.
For this situation (\ref{eq:a2}), the general trial ansatz~$\Psi^{\{0\}}_\infty(y)$~(40) adopts the special
form
\begin{equation}
  \label{eq:a3}
  \Psi^{\{0\}}_\infty(y)\Rightarrow \overset{\circ}{\Psi}{}^{\{0\}}_\infty(y) =
  \frac{1}{2\sqrt{\ln 2}}\cdot\frac{1}{\cosh\frac{y}{2}}\ .
\end{equation}
Of course, this wave function~$\overset{\circ}{\Psi}{}^{\{0\}}_\infty(y)$ is normalized to
unity
\begin{equation}
  \label{eq:a4}
  \int_0^\infty dy\,y\left(\overset{\circ}{\Psi}{}^{\{0\}}_\infty(y) \right)^2 = 1
\end{equation}
since the normalization condition~(41) is satisfied by \emph{all} members of the trial
set $\Psi^{\{0\}}_\infty(y)$~(40). 

Concerning now the energy ($\overset{\circ}{\EE}{}^{\{0\}}_\infty$, say) due to the
present groundstate ansatz~$\overset{\circ}{\Psi}{}^{\{0\}}_\infty(y)$~(A.3), it should be
clear that the general result~$\EE^{\{0\}}_\infty(g)$~(49) becomes specified to
\begin{equation}
  \label{eq:a5}
  \EE^{\{0\}}_\infty(g)\Rightarrow \overset{\circ}{\EE}{}^{\{0\}}_\infty = 
\frac{e^2}{4\aB}\frac{\left(\overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm pot,\infty}
  \right)^2}{ \overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm kin,\infty} }\ .
\end{equation}
Here the electrostatic coefficient~$\overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm
  pot,\infty}$ is to be deduced from its general form~(44b) as
\begin{equation}
  \label{eq:a6}
  \varepsilon^{\{0\}}_{\rm  pot,\infty} \Rightarrow \overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm pot,\infty}=
  \int_0^\infty dy\,y\left(\frac{d \overset{\circ}{\A}{}^{\{0\}}_\infty(y) }{dy} \right)^2
\end{equation}
and similarly the kinetic coefficient~$\overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm
  kin,\infty}$ is a specialization of~$\varepsilon^{\{0\}}_{\rm  kin,\infty}$~(44a):
\begin{equation}
  \label{eq:a7}
    \varepsilon^{\{0\}}_{\rm  kin,\infty} \Rightarrow  \overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm kin,\infty} =
  \int_0^\infty dy\,y\left(\frac{d\, \overset{\circ}{\Psi}{}^{\{0\}}_\infty(y) }{dy}
  \right)^2\ .
\end{equation}
Thus, one substitutes that special value for~$g$~(A.2) in the result~(50)
for~$\varepsilon^{\{0\}}_{\rm  kin,\infty}$ and obtains
\begin{equation}
  \label{eq:a8}
\overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm kin,\infty} = \frac{\ln2+\frac{1}{2}}{12\ln 2}
= 0.143445 \ldots
\end{equation}

In a quite similar way, one obtains also the value of the electrostatic
coefficient~$\overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm pot,\infty}$~(A.6), namely by
substituting the special value~$\overset{\circ}{g}$ in equation~(62) which yields
\begin{equation}
  \label{eq:a9}
  \overset{\circ}{\varepsilon}{}^{\{0\}}_{\rm pot,\infty} = \frac{\frac{1}{2}-\left(1-\ln
      2 \right)}{\left(\ln 2 \right)^2 } = 0.402010 \ldots
\end{equation}
Consequently, the final result~(A.5) is
\begin{equation}
  \label{eq:a10}
  \overset{\circ}{\EE}{}^{\{0\}}_\infty \simeq
  -\frac{e^2}{4\aB}\cdot\frac{\left(0,4019\right)^2}{0,1434} = -\frac{e^2}{4\aB}\cdot
  1,1264 = -7,66278\,[\text{eV}]\ .
\end{equation}
This prediction for the groundstate energy is \emph{slightly higher} than the minimal
value obtainable in our set of trial ans\"atze~(40), cf.~\textbf{Fig.2}, and therefore
confirms the correctness of our numerical minimalization program.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> macros_stary.tex <==


%    'A   ein Strich (Apostroph) links oben
\newcommand{\slo}[1]{\,'{\!#1}}

%	 {p}                                                
%      A_blah  geschweifte Klammer links oben rechts unten roman index
%
\newcommand{\gkloi}[3]{\, {}^{\{\mathrm{#1}\}}{\!{#2}}_\mathrm{#3}}

%	 {p}                                                
%      A_blah  geschweifte Klammer links oben
%
\newcommand{\gklo}[2]{\, {}^{\{\mathrm{#1}\}}{\!{#2}}}

% (p)
%    A    runde Klammer mit roman links oben     
%
\newcommand{\rrklo}[2]{\, {}^{(\mathrm{#1})}{\! {#2} }}
% (p)
%    A    runde Klammer mit \sf (ohne Serifen) links oben     
%
\newcommand{\srklo}[2]{\, {}^{({\sf #1})}{\! {#2} }}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

